Generic 3D Representation via Pose Estimation and Matching

Though a large body of computer vision research has investigated developing generic semantic representations, efforts towards developing a similar representation for 3D has been limited. In this paper, we learn a generic 3D representation through solving a set of foundational proxy 3D tasks: object-centric camera pose estimation and wide baseline feature matching. Our method is based upon the premise that by providing supervision over a set of carefully selected foundational tasks, generalization to novel tasks and abstraction capabilities can be achieved. We empirically show that the internal representation of a multi-task ConvNet trained to solve the above core problems generalizes to novel 3D tasks (e.g., scene layout estimation, object pose estimation, surface normal estimation) without the need for fine-tuning and shows traits of abstraction abilities (e.g., cross-modality pose estimation). In the context of the core supervised tasks, we demonstrate our representation achieves state-of-the-art wide baseline feature matching results without requiring apriori rectification (unlike SIFT and the majority of learned features). We also show 6DOF camera pose estimation given a pair local image patches. The accuracy of both supervised tasks come comparable to humans. Finally, we contribute a large-scale dataset composed of object-centric street view scenes along with point correspondences and camera pose information, and conclude with a discussion on the learned representation and open research questions.

==> intro_backup1.tex <==
%-----------------------------------


\section{Introduction}
\label{sec:intro}
A representation performs the task of converting visual information to a mathematical form (often a vector). This mathematical form is expected to encode the information required for solving the task it was devised for, and ideally, generalize to related problems.
While a considerable number of existing works have explored the possibility of forming generic semantic representations~\cite{decaf,razavian2014cnn,bengio2013representation}, transfer learning~\cite{Trzcinski,raina2007self,quattoni2008transfer}, and initialization strategies of ConvNets~\cite{cmuvideo,LSM2015,doersch2015unsupervised} useful for scaling recognition tasks, an equivalent representation for 3D is yet to be proposed.
We take a step towards developing a generic 3D representation, that 1) can solve novel 3D problems without the need for fine-tuning the representation, and 2) is capable of certain abstract generalizations in the 3D context (e.g., reason about pose similarity between two drastically different objects).

But, how one could learn such a generalizable representation? Cognitive studies suggest living organisms can perform cognitive tasks for which they have not received supervision by supervised learning of other foundational tasks~\cite{twokitten,smith2005development,rader1980nature}.  Learning the relationship between visual appearance and changing the vantage point (self-motion) is among the first visual skills developed by infants and play a fundamental role in developing other skills, e.g., depth perception. 
A classic experiment~\cite{twokitten} showed a kitten that was deprived from self-motion experienced fundamental issues in 3D perception, such as failing to understand depth when placed on the Visual Cliff~\cite{visualcliff}. Later studies~\cite{rader1980nature} argued this finding was not, at least fully, due to motion intentionality and the supervision signal of self-motion was indeed a crucial elements in learning basic visual skills.
%(young infants prior to development of motor skills, that would allow them to practice motion intentionality, were found to respond to visual cliff through an increase in their heart rate\todo{removal candidate: the sentence in parentheses}).
What these experiments essentially suggest are: 1) by receiving supervision over a certain proxy task (in this case, visual perception of self-motion), other tasks (depth understanding) can be solved sufficiently without requiring an explicit supervision, 2) some vision tasks are more foundational than others (e.g., self-motion perception vs depth understanding).

			\begin{figure}
				\centering
				\includegraphics[width=1\columnwidth]{figs/teaser_9.pdf}
				\caption{\scriptsize{\textbf{Learning a generic 3D representation}: we develop a supervised joint framework for camera pose estimation and wide baseline matching. We then show the internal representation of this framework can be used as a 3D representation generalizable to various 3D prediction tasks.\vspace{0pt}}}
				\label{fig:teaser}
			\end{figure} 

Inspired by the above discussion, we develop a supervised framework where a ConvNet is trained to perform 6DOF camera pose estimation. This basic task allows learning the relationship between an arbitrary change in the viewpoint and the appearance of an object/scene-point. One property of our approach is performing the camera pose estimation in a object/scene-centric manner: the training data is formed of image bundles that show the \emph{same point of an object/scene} while the camera moves around (i.e., it fixates - see the figure \ref{fig:datacol} (c)). This is different from existing video+metadata datasets~\cite{kitti}, the problem of Visual Odometry~\cite{nister2004visual,kitti}, and recent works on ego-motion estimation~\cite{LSM2015,dinesh}, where in the training data, the camera moves independent of the scene. Our object/scene-centric approach is equivalent to allowing a learner to focus on a physical point while moving around and observing how the appearance of that particular point transforms according to viewpoint change. Therefore, the learner receives an additional piece of information that the observed pixels are indeed showing the same object, giving more information about how the element looks under different viewpoints and providing better grounds for learning visual encoding of an observation. %while 
%The scene-independent motion scenario~\cite{kitti} is different and provides better bases for inferring camera pose change (e.g., visual odometry) in dynamic environments. 
%\todo{is this true? Should we remove the second part of the sentence?}. 
Infants also explore object-motion relationships~\cite{smith2005development} in a similar way as they hold an object in hand and observe it from different views. %\todo{@Pulkit: is this true or significant? reference?} \todo{a more concrete support for why object-centric is better?}\todo{removal candidate: last 3 lines}

Our dataset also provides supervision for the task of wide baseline matching, defined as identifying if two images/patches are showing the same point regardless of the magnitude of viewpoint change. Wide baseline matching is also an important 3D problem and is closely related to object/scene-centric camera pose estimation: to identify whether two images could be showing the same point despite drastic changes in the appearance, an agent could learnt how viewpoint change impacts the appearance. Therefore, we perform our supervised training in a multitask manner to simultaneously solve for both wide-baseline matching and pose estimation.
This has the advantages of learning a single representation that encodes both problems. In experiments section (\ref{sec:joint}), we show it is possible to have a single representation solving both problems without a performance drop compared to having two dedicate representations. This provides practical computational and storage advantages. Also, training ConvNets using multiple tasks/losses is desirable as it has been shown to be better regularized~\cite{Xu2015,girshick15fastrcnn,weston2012deep}.\footnote{Though visual matching/tracking is also one of the early developed cognitive skills\cite{infanttracking}, we are unware of any studies investigating its foundational role in developing visual perception. Therefore, we presume (and empirically observe) that the generality of our 3D representation is mostly attributed to the camera pose estimation component.} 

We train the ConvNet (siamese structure with weight sharing) on patch pairs extracted from the training data and use the last FC vector of one siamese tower as the 3D representation (see figure~\ref{fig:teaser}). We will empirically investigate if this representation can be used for solving novel 3D problems (we evaluated on scene layout estimation, object pose estimation, surface normal estimation), and whether it can perform any 3D abstraction (we experimented on cross category pose estimation and relating the pose of synthetic geometric elements to images).



\textbf{Dataset}:
We developed an object-centric dataset of streetview scenes from the cities of Washington DC, NYC, San Francisco, Paris, Amsterdam, Las Vegas, and Chicago, augmented with \emph{camera pose} information and \emph{point correspondences} (with $>$half a billion training data points). We release the dataset, trained models, and an online demo at \textcolor{blue}{\url{http://3Drepresentation.stanford.edu/}}.

\textbf{Novelty in the Supervised Tasks}:
Independent of providing a generic 3D representation, our approach to solving the two supervised tasks is novel in a few aspects. There is a large amount of previous work on detecting, describing, and matching image features, either through a handcrafting the feature~\cite{sift,surf,mikola,mser,alahi2012freak,pernoa_survey} or learning it~\cite{simonyan,matchnet,cvpr15,balntas2016pn,zbontar2015computing,simo2015discriminative,cnnunsup}. Unlike the majority of such features that utilize pre-rectification (within either the method or the training data), we argue that rectification prior to descriptor matching is not required; our representation can learn the impact of viewpoint change, rather than canceling it (by directly training on non-rectified data and supplying camera pose information during training). Therefore, it does not need an apriori rectification and is capable of performing wide-baseline matching at the descriptor level. We report state-of-the-art results on feature matching. 
Wide baseline matching has been also the topic of many papers~\cite{pritchett1998wide,tell2002combining,goedeme2004fast,xiao2003two,zhang2012tilt} with the majority of them focused on leveraging various geometric constraints for ruling out incorrect `already-established' correspondences, as well as a number of methods that operate based on generating exhastive warps~\cite{morel2009asift} or assuming 3D information about the scene is given~\cite{wu20083d}. In contrast, we learn a descriptor that is supervised to internally handle a wide baseline in the first place.

In the context of pose estimation, we show estimating a 6DOF camera pose given only a pair of local image patches, and without the need for several point correspondences, is feasible. 
This is different from many previous works \cite{rome,zissermanBook,visualsfm,song2013parallel,badino2013visual,chen2011city,kitti} from both visual odometery and SfM literature that perform the estimation through a two step process consisting of finding point correspondences between images followed by pose estimation. Koser and Koch~\cite{koser2008differential} also demonstrate pose estimation from a local region, though the plane on which the region lies is assumed to be given. The recent works of~\cite{LSM2015,dinesh} supervise a ConvNet on the camera pose from image batches but do not provide results on matching and pose estimation.  We report a human-level accuracy on this task. 

 




\textbf{Existing Unsupervised Learning and ConvNet Initialization Methods}:
The majority of previous unsupervised learning, transfer learning, and representation learning works have been targeted towards semantics~\cite{decaf,razavian2014cnn,sermanet2013overfeat,doersch2015unsupervised,tarr1994computational}. It has been practically well observed~\cite{decaf,razavian2014cnn} that the representation of a convnet trained on imagenet~\cite{krizhevsky2012imagenet} can generalize to other, mostly semantic, tasks. A number methods investigated initialization techniques for ConvNet training based on unsupervised/weakly supervised data to alleviate the need for a large training dataset for various tasks~\cite{cmuvideo,doersch2015unsupervised}. Very recently, a few methods~\cite{LSM2015,dinesh} investigated using motion metadata associated with videos (KITTI dataset~\cite{kitti}) as a form of supervision for training a ConvNet. However, they either do not investigate developing a 3D representation or intent to provide initialization strategies that are meant to be fine-tuned with supervised data for a desired task. In contrast, we investigate developing a generalizable 3D representation, perform the learning in an object-centric manner, and evaluate its unsupervised performance on various 3D tasks without any fine-tuning on the representation. We experimentally compare against the related recent works that made their models available~\cite{LSM2015,cmuvideo}.
%\todo{@Pulkit: you're more familiar with the ICCV papers, especially Dinesh's and yours. Can you pronounce the difference between ours and those a bit more strongly here? especially Dinesh's since we dont have comparisons with them (no model). Or is it good as-is?}



The main contributions of this paper can be summarized as:\\ 
I) A generic 3D representation with empirically validated abstraction and generalization advantages. \\
II) A joint learned descriptor for wide baseline matching and camera pose estimationat at the level of local image patches. \\
III) A large-scale object-centric dataset of streetview scenes including camera pose and correspondence information. \\
  




%One of the most fundamental aspects of our 3D world is that, as an observer changes its vantage point, objects in the scene undergo a viewpoint transformation. This gives rise to three basic and closely related problems in computer vision: 1) how to find correspondences between images taken from different viewpoints? 2) what is the relative observer's pose between the two images? 3) how to infer shape information about the object using motion? Even though these problems are closely tangled, they have been commonly treated separately, mostly due to the facts that either the essential powerful learning tools were not developed or the required large-scale multi-task training data was not available. We turn this around by learning a joint representation for these tasks using a multi-task Convolutional Neural Network (ConvNet) and an unprecedented ultra-scale dataset. Such a joint representation has several fundamental advantages, such as:

 
%\textbf{A natural approach and induction of abilities}: with the problems being very cognate, it is logical to address them jointly. This will allow the tasks to share information and possibly induce abilities. That way, a function that is well learned for one of the problems can be potentially induced on another when applicable, through the shared information. We will show the aforementioned core problems naturally share a great deal of information. Our joint representation can be perceived to be be simultaneously equivariant and invariant with respect to all three problems.

%\noindent
%\textbf{Better regularization and generalization:} joint representations are better regularized as they receive a loss from multiple and different tasks\cite{Xu2015,Girshick15,Ghifary15}. Compared to single-task counterparts, a representation that has to simultaneously solve several problems is less likely to overfit to one. We will experimentally show this in Section~\ref{sec:results}. 

%\noindent
%\textbf{Computation and storage:} we show that all the three tasks can be performed a single descriptor which leads to significant storage and computation advantages ($\sim$3X) as all the three tasks can be solved with one computation. 
%we will prove that the tasks heavily share information and show that a single joint descriptor can store the required information for solving all three problems and yet performs comparable to or better than its dedicated (i.e., single-task) counterparts. This has clear storage and complexity advantages ($\sim$3X) since all three tasks can be solved with one computation. 

%Besides arguing for addressing these core problems jointly, we put forth two other new paradigms for the tasks of matching and camera pose estimation:


%In the context of matching (finding correspondences), initially hand crafted features, most notably SIFT, were devised~\cite{sift,rootsift}. Later, feature learning that attempted performing the same task through end-to-end learning was explored~\cite{simonyan,cvpr15,cnnunsup,brown}. Even though both of these approaches yield promising results, they all employ a common paradigm: they attempt to find  correspondences by canceling the impact of viewpoint change and seeking a \emph{view-invariant} space. In other words, they look at viewpoint change as an adversary whose impact should be removed. This rather complicated cancellation task is usually delegated to key-point/region detectors, e.g. MSER~\cite{MSER}, SIFT~\cite{sift,mikola,pernoa_survey}.


%We question this common paradigm and argue that for ultimately solving wide baseline matching, pose change information should be in fact utilized rather than canceled. Our approach is based upon the following argument: though viewpoint shift can change the appearance of one object  in an infinite number of ways, yet the change is very constrained; in other words, the shape of an object cannot turn into an arbitrary form just because of viewpoint shift. 
%For instance, as humans, we can easily identify whether two things that immediately look very different are actually the same thing and the drastic appearance change is merely due to viewpoint difference. %remove 
%The fact that this problem is heavily constrained implies that it can be effectively learned. 
%This is also intuitive from the cognitive perspective since some studies suggest human brain does not form a single canonical rectified view~\cite{tarr1989mental,shepard1971mental}. %Instead, we reason about the pose and utilize it. %remove
%Inspired by our initial discussion on the feasibility of learning the impact of viewpoint change, 
%Therefore, we avoid the aprior rectification step and learn a local feature descriptor that can determine whether \emph{two very different looking patches} could be showing the same portion of an object. 
%We attempt learning a local feature descriptor capable of performing wide baseline handling without an aprior rectification step and 
%We also train a pose regressor that can reason about the camera pose change. % REMOVE?

%that’s why finding correspondences and identifying the relative pose happen almost simultaneously for us. %remove
%In addition, understanding the pose at the low level of local features has additional advantages which makes this approach a worthwhile effort.


%In our approach, we put this statement into question: can we learn a local feature descriptor capable of performing wide baseline matching without the need of any a-priori rectification or key-point detector? More specifically, we address two core problems: 1) Learn pose estimation between two local feature patches given only the raw pixels with no keypoints or preprocessing. Once we prove this is feasible, 


%In the context of camera pose estimation, the dominating approach is to first find a set of point correspondences between images, and then form the fundamental matrix and follow standard structure-from-motion procedure~\cite{rome,zissermanBook,visualsfm}. Thus, the first problem is assumed to be at least partially solved which makes any reasoning on pose conditional on having point correspondences already. 

%Inspired by our above argument on feasibility of learning pose-caused appearance change, we again question the traditional structure-from-motion paradigm and show that it is indeed possible to estimate the relative camera pose without having correspondences, even given only two local features (patches). 
%It has been in fact well studied that pose estimation can be accomplished using other information, e.g. common vanishing points~\cite{vanish_calib,zissermanBook} or local texture deformation~\cite{jitendra_texture,zhang2011tilt,white2006combining}, though these techniques are not usually employed in practice because extracting their required input, e.g. vanishing points, are themselves open problems. 
%Our approach to camera pose estimation is also the philosophical basis for our solution to finding correspondences since it verifies that extracting any pose information given merely a pair of local features is feasible.

 %The second task would be unlikely to be feasible if the first one turned out to be infeasible. We will show both of these can be well achieved.



%We employ a strictly data-driven and feature learning based approach to this problem. In this context, our goal could be potentially accomplished in two ways: 1) adopt a learning technique and provide it with sufficient training data composed of wide baseline correspondences (rather than rectifying them a priori) and hope that the model will perform satisfactorily,
%2) or better, first specifically develop a model that is capable of reasoning about pose, then employ it for learning a feature which can perform wide baseline matching. We investigate both of these approaches and share our insights. 


%The above learning problem is notably more complex than the conventional approaches.
%``pose-normalized'' feature learning as viewpoint change brings a lot of variance to the appearance space. 
%Given this reason and the data hungry nature of Convolutional Neural Networks (ConvNet), a massive amount of training data would be essential. 
%We show how we automatically built an ultra-scale (over half a billion data points and counting), diverse, and pose-rich dataset allowing us to perform the learning job in a fully supervised manner \emph{without any manual annotation}. 
%The dataset essentially shows 3D points seen in streetview images from different viewpoints and preserves the viewpoint information of the camera and shape information of the object. The dataset, trained ConvNet, a demo, and the reported results on the test set are available at \url{URL}. 

%We address the aforementioned problem in the context of local features (patches) because of their broad usage and practical advantages.
%, such as occlusion handling, computational efficiency, and better generalization compared to holistic features. 
%We train a multi-task ConvNet with a Siamese structure for performing camera pose regression and wide baseline matching given two local patches. The last layer of one of the towers of this siamese network is then adopted as the final local feature descriptor (see Figure \ref{fig:teaser}) that is robust to drastic camera pose changes without any rectification and also jointly encodes matching (appearance), shape and relative camera pose information. We could perform shape estimation\footnote{We adopt surface normals as our notion of shape and refer to them interchangeably.} through adding this task to the ConvNet as well; however, we made the key observation that the ConvNet trained for the two tasks of matching and pose estimation interestingly self-supervises itself into surface normals. That is another evidence for strong information sharing among these tasks. Therefore, we infer the surface normals without adding it as a separate task to the network.


%We will present that upon adopting the above new paradigms and utilizing our unprecedented training data, but ironically using ConvNets with the most straightforward architectures all of existing appearance features are outperformed.%., but also local-feature-level pose estimation is made possible. 
%We will also make efforts towards understanding the internal pose representation of the ConvNet and hypothesize that it has internally recreated the fundamental concepts of surface normals and vanishing points without receiving any explicit supervision for them. 




==> nonSFN.tex <==

\section{Joint Feature Learning}
\label{sec:joint}
We investigated different aspects of joint learning the representation and information sharing among the two supervised tasks in Tables~\ref{tab:trans} and ~\ref{tab:joint-net}. To quantify the amount of information shared among the matching and pose estimation tasks, we trained a single-task network dedicated to each problem; their error for their respective task is reported in ``Direct" row of the Table~\ref{tab:trans}. ``Transduction"  provides the error rate when a linear classifier was trained on the frozen representation of one task to solve the other task. The fact that the Transduction setup achieves a reasonable performance suggests the two problems have a great deal of shared information in their representations. Table~\ref{tab:joint-net} compares the performance of single vs multi-task networks. The multi-task network performs comparable to its dedicated counterparts showing it encoded both problems with no performance drop.

\begin{table*}
	%\caption{\scriptsize{Illustrating the benefits the jointly learning features for camera pose estimation and patch matching. The results for patch matching are reported as FPR @95\% recall and for pose estimation in degrees.}}
	\parbox{.60\linewidth}{
		\centering
		\caption{\scriptsize{Information Sharing Among Supervised Tasks}}
		\vspace{0pt}
		\scalebox{0.65}{
			\begin{tabular}{c|c|c}
				& Matching (FPR) & Pose (Error)  \\
				\hline
				Direct& 23.54\% & $16.58\degree$\\
				\hline
				Transduction & 30.06\% & 24.50 $\degree$\\
				\hline
				Chance & 95\% & 90 $\degree$ \\
				\hline
			\end{tabular}}
			\label{tab:trans}
		}
		\hfill \hspace{-0.3mm}
		\parbox{.40\linewidth}{
			\centering
			\caption{\scriptsize{Joint vs Individual Learning}}
			\vspace{0pt}			
			\scalebox{0.65}{
				\begin{tabular}{c|c|c}
					& Matching (FPR) & Pose (Error)  \\
					\hline
					Pose-Net & - & $16.58\degree$\\
					\hline
					Matching-Net & 23.54\% & -\\
					\hline
					Joint-Net & 23.0\% & 17.78 $\degree$ \\
					\hline
				\end{tabular}
			}\label{tab:joint-net}}
		\vspace{0pt}
	\end{table*}
	






\section{Brown et al. Benchmark.}
%\label{sec:brown} 
We evaluated the performance of our representation on the benchmarks of Brown et al.~\cite{brown} and Mikolajczyk \& Schmid~\cite{mikola} (next subsection). Compared to our dataset, these benchmarks mostly include narrower baselines (except for a subset of~\cite{mikola}), and therefore, do not pronounce wide baseline handling abilities; our method also sees more training data than the baselines. However, these benchmarks would reveal 1) if our representation was performing well only on street view scenery, and 2) if wide baseline handling capability was achieved at the expense of lower performance on small baselines. 

We compared our results with six baselines, including Zagoruyko \& Komodakis's~\cite{cvpr15} and MatchNet~\cite{matchnet}, against their most similar descriptor dimensionality (512) and network architecture to ours. For this experiment, we mixed our training dataset with the corresponding training split of Brown's (see Table~\ref{tab:brown}). 
Our representation outperforms the baselines, except for two splits from the Yosemite National Park that are substantially foliage covered (for which we speculate that the foliage coverage is reason since our ConvNet is mostly agnostic with respect to foliage as trees are uninformative for matching and pose in street view scenery).





\begin{table*}
	%\caption{Evaluation on Brown's Benchmark~\cite{brown} and Mikolajczyk \& Schmid's~\cite{mikola} benchmark.\vspace{-2pt}}
	\label{tab:joint}
	\parbox{.58\linewidth}{
		\centering		
		\caption{\scriptsize{Evaluations on Brown's Benchmark~\cite{brown}. FPR@95 ($\downarrow$) is the metric.}}% Last two splits are foliage covered.}}
		\label{tab:brown}
		\vspace{0pt}
		\scalebox{0.65}{
			\begin{tabular}
				{ @{}c@{} | @{}c@{} | @{}c@{} | @{}c@{} | @{}c@{} | @{}c@{} | @{}c@{} | @{}c@{} | @{}c@{} }
				{\bf Train } & {\bf{ Test }} & {  \scriptsize{ MatchNet }} & {{ \scriptsize{ Zagor. }}}& {{\scriptsize{ Simonyan~  }}}& {{\scriptsize{ Trzcinski }}} & {{ \scriptsize{ Brown }}} & {{ \scriptsize{ Root-SIFT }}} & {{\bf \scriptsize{ Ours}}}   \\ 
				{ } & { } & ~\cite{matchnet} & \scriptsize{siam~\cite{cvpr15}} & ~\cite{simonyan} & ~\cite{Trzcinski}  &  ~\cite{brown} &  ~\cite{rootsift}  & { }   \\ \hline
				Yos & ND  & 7.70 & 5.75 & 6.82 & 13.37 & 11.98 & 22.06 & \textbf{4.17} \\
				Yos & Lib  & 13.02 & 13.45 & 14.58 & 21.03 & 18.27 & 29.65 & \textbf{11.66} \\
				Lib & ND  & 4.75 & 4.33 & 7.22 & 14.15 & N/A & 22.06 & \textbf{1.47} \\ 
				ND & Lib  & 8.84 & 8.77 & 12.42 & 18.05 & 16.85 & 29.65 & \textbf{7.39} \\ \hline
				Lib & Yos  & 13.57 & 14.89 & \textbf{11.18} & 19.63 & N/A & 26.71 & 13.78 \\ 
				ND & Yos  & 11.00 & 13.23 & \textbf{10.08} & 15.86 & 13.55 & 26.71 & 12.30 \\\hline
				\multicolumn{2}{c|}{{mean}}  & 9.81  & 10.07 & 10.38 & 17.01 & 15.16  & 26.14 & \bfseries{8.46} \\
			\end{tabular}}
		}
		\hfill \hspace{0.01mm}
		\parbox{.42\linewidth}{
			\centering
			\vspace{0pt}
			\caption{\scriptsize{Evaluation on Mikolajczyk \& Schmid's~\cite{mikola}. The metric is mAP($\uparrow$).}}
			\label{tab:Mikola}
			\vspace{11pt}
			\scalebox{0.65}{
				\begin{tabular}{ c | c  c  c  c  c }
					\textbf{\footnotesize{Transf.}} & \multirow{2}{*}{\textbf{\small{1}}} & \multirow{2}{*}{\textbf{\small{2}}} & \multirow{2}{*}{\textbf{\small{3}}} & \multirow{2}{*}{\textbf{\small{4}}} & \multirow{2}{*}{\textbf{\small{5}}}\\
					\textbf{\footnotesize{Magnitude}} & & & & & \\ \hline
					\footnotesize{SIFT~\cite{sift}} &  40.1 &  28.0 & 24.3 & 29.0 &  17.1 \\
					\footnotesize{Zagor.~\cite{cvpr15}} & 43.2 & 37.5 & 29.2 & 28.0 & 16.8 \\ 
					\footnotesize{Fischer et al~\cite{cnnunsup}} & 42.3 & 33.9 & 26.1 & 22.1 & 14.6 \\ \hline
					%MSER siam-SPP-l2 & 48.12 & 38.7 & 36.31 & 35.51 & 18.36 \\ 
					%MSER 2ch-deep & 45.89 & 39.2 & 33.42 & 42.12 & 29.23 \\ 
					%MSER R 2ch-2stream & 47.05 & 42.15 & 37.09 & 37.05 & 27.68 \\
					\footnotesize{Ours-rectified} & 46.4 & \textbf{41.3} & 29.5 & 23.7 & 17.9 \\ 
					\footnotesize{Ours-unrectified} & \textbf{51.4} & 37.8 & \textbf{34.2} & \textbf{30.8} & \textbf{20.8} \\
				\end{tabular}}
			}
			\vspace{0pt}
		\end{table*}
		
		
		
		%-----------
		
		\subsubsection{Mikolajczyk \& Schmid Benchmark.}
		The evaluation results on the benchmark of Mikolajczyk \& Schmid~\cite{mikola} are provided in Table~\ref{tab:Mikola} using the standard protocol~\cite{mikola,cvpr15}. Following~\cite{cvpr15,cnnunsup}, we performed the matching on MSER features. The last two rows show our results on the MSER patches with and without rectification (i.e., skipping MSER rectification). Our representation outperforms the baselines in both cases, while not performing the rectification actually improves the performance. 


\section{Dataset and Data Collection Details}
Our dataset was collected from a broad geographical area spanning multiple cities. Some representative city locations from which data was collected are shown in Figure~\ref{fig:datacoverage}.  

\begin{figure*}
	\centering
	\includegraphics[width=1\textwidth]{figs/dataset_coverage_v1.pdf}
	\caption{\scriptsize{Some of the areas from which we have collected our dataset.}}
	\label{fig:datacoverage}
\end{figure*}

Sample images from our dataset that were used for training the pose estimation and patch matching network are shown in Figures~\ref{fig:sampledata1},\ref{fig:sampledata2}. Each row in the figure shows a single target location from different viewpoints. The target location is marked with a red dot. 

\begin{figure*}
	\centering
	\includegraphics[width=1\textwidth]{figs/sample_data2.pdf}
	\caption{\scriptsize{Sample images from our dataset. Each row shows one image bundle showing one target. The marker is on the center pixel and should show the target point. The columns show different views.}}
	\label{fig:sampledata1}
\end{figure*}


\begin{figure*}
	\centering
	\includegraphics[width=1\textwidth]{figs/sample_data1.pdf}
	\caption{\scriptsize{Sample images from our dataset. Each row shows one image bundle showing one target. The marker is on the center pixel and should show the target point. The columns show different views.}}
	\label{fig:sampledata2}
\end{figure*}






\subsection{Pixel Alignment and Pruning}
The data collection system required integration of multiple resources, including GPS from street view, elevation maps, and 3D models. Any slight inaccuracy in the metadata or 3D models can cause a pixel misalignment in the collected images. Therefore, we performed the following pose-processing procedure to cancel some of these errors.


We wish to verify if the center of images in a bundle show the same physical target and adjust them if necessary. 
The collected image bundles can show large (often $>100\degree$) viewpoint changes, while the existing registration methods do not handle such large angular changes in unconstrained scenes. %(see Figure~\ref{fig:alignment}, first and second column).
To solve this issue, we utilize the metadata again: 
we extract the relative pose of the cameras to the desired physical point's surface normal (acquired from the 3D models). Then a homography transformation is applied to project one patch in the bundle onto another in a way that the local image planes on which the desired physical point lies are parallel. This cancels the perspective transformation caused by the baseline change (see `Warped' in Figure~\ref{fig:alignment}).
Thus, the registration transformation between the two rectified images can be effectively approximated by a similarity transformation.
To avoid a quadratic complexity with respect to the number of images, we select the most frontal view for each target point and align the rest of the images of the target with respect to it.

Since the patches often show non-planarity, we found employing a nonrigid transformation (we used SIFT flow~\cite{siftflow}) for registration of the rectified patches to be more robust. We use RANSAC to fit a similarity transformation to the resulting flow field and apply the inverse of the rectification transformation to find the translation vector which should be applied on the original image to perform the alignment~(see `Aligned' in Figure~\ref{fig:alignment}). We use only the translation component for performing the alignment since we want to preserve the original camera rotation information to use it in training.
Finally, to remove the remaining unreliable and occluded patches, we extract two registration metrics (Structural Similarity Index which measures the pixel similarity among registered images, and magnitude of the estimated transformation) and threshold the dataset based on them (see `Occluded' in Figure~\ref{fig:alignment}-b).

\begin{figure}
	\centering
	\includegraphics[width=1\columnwidth]{figs/alignment_fig_opt4.pdf}
	\caption{\scriptsize{\textbf{Pixel alignment process} for two sample targets. Blue arrow shows the adjustment vector between the initial and updated position of the center. (b) shows a case with occlusion (view 4).\vspace{0pt}}
		%(on the left and right). 
		%The first column illustreetviewates streetview images with the center pixel aligned using on the camera metadata and 3D building models, which shows misalignment inaccuracies because of imperfect metadata and 3D models. The second column shows the cropped center patch. Ideally, the marker should be grounded on the same physical point, while some misalignment can be seen. The third and forth column show the patch after rectification based the surface normal and the rectified patches after registration, respectively. The fifth column shows the registered warped patch after application of the inverse warping. Notice that the center marker is now perfectly grounded on a physical point. 
	}
	\label{fig:alignment}
\end{figure}

\subsection{Noise Statistics}
A user study through Amazon Mechanical Turk was performed to quantify the amount of noise in the final dataset. 15124 random pairs of matching patches from the dataset were annotated by three Turkers to identify if they have at least $25\%$ overlap in their content, and if not, what the reason was. Also, to quantify the magnitude of pixel misalignment, they were asked to click on the pixel in the $2^{nd}$ patch which corresponds to the center pixel of the $1^{st}$ patch. 

About $68\%$ of the pairs were found to have at least $25\%$ overlap (by majority voting). For the subset with less than $25\%$  overlap, the originating issues were identified as: $49.5\%$ due to inaccuracies in meta-data and 3D models, $27.7\%$ due to tree occlusion, $16.5\%$ due to other occlusions, and $6.1\%$ other reasons. In heavily tree occluded areas (e.g., Washington D.C. suburb), the percentage of matching pairs reduced to $58\%$. Such areas can be easily avoided by geo-fencing (e.g., by collecting data from downtowns since they show more buildings than trees compared to suburbs). 

The mean and standard deviation of the magnitude of misalignment (defined as the magnitude of the vector connecting the center of the $2^{nd}$ patch to the pixel location where the Turkers clicked) was 16.12 ($\approx11\%$ of patch width) and 11.55 pixels, respectively. 

In our training dataset, we did not perform any manual filtering or geo-fencing on top of the automatically collected data since the amount of noise appeared to be within the robustness tolerance of ConvNets as their training converged and well performed on the carefully filtered test set.






==> sfnnyu.tex <==
\section{Surface Normal Estimation}

Estimating surface normals is a fundamental problem in 3D computer vision. We evaluated the usefulness of the representation learned by our method for surface normal estimation on the standard NYU2 benchmark \cite{silberman2012indoor,eigen2015predicting,Wang15}. The dataset contains 795 training images and 654 testing images. 

In this work, our goal is not to develop the best method for a specific task,  but rather to investigate how useful are features learned by training for pose-estimation for various 3D tasks without the requirement for fine-tuning. For this task, we employed two methods to read the surface normal value out of the representation of an image/patch: a linear classifier and nearest neighbors. While running our experiments, we noticed that the surface normal estimation in the NYU dataset is heavily biased as most pixels belong to one of the three categories of ceiling, floor, and walls. This inevitably means that the prediction results would be dominated by performance on such categories. In order to account for this, we propose the use of reporting binned errors. The binned errors are calculated by first binning pixel wise surface normals into 20 bins (in a manner similar to \cite{Wang15}) and calculating the error within each bin. Then we calculate the average statistics such as the mean or the median across the bins. The idea of using binned error is similar to the idea of reporting mean of the class accuracies in classification tests. In addition to this setup, we also report numbers according to the standard benchmark evaluation of pixelwise median error and the percentage of pixels that were within $11.5^{o}, 22.5^{o}$ and $30^{o}$ respectively. 

\subsection{Prediction via Linear Classification} 
In previous works, such as \cite{Wang15,cmuvideo}, coarse surface normals were estimated by predicting normals on a 20x20 spatial grid. The normal of each grid block is predicted by solving a 20 way classification problem, where the 20 classes correspond to 20 pre-calculated surface normal clusters. The final estimate is provided by up sampling this 20x20 grid into the full image resolution.  

Following a similar experimental setup, we first report the accuracy of predicting surface normals on 20x20 grids. We trained a linear classifier on top of our representation as well as the methods of \cite{LSM2015,cmuvideo} and AlexNet trained for ImageNet. We report the classification accuracy in individual grid locations and the mean/median angular error in the estimated surface normals. The angular error is calculated as the angular distance between the predicted and ground truth surface normal clusters. We report accuracies with and without binning in Table \ref{table:nyubin} indicating that our representation outperforms AlexNet and \cite{LSM2015,cmuvideo}. 

\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
\begin{center}
\caption{\scriptsize{Evaluation of surface normal estimation on the NYU2 dataset using the 20-way classification setup. We trained a linear classifier on top of the representations to perform the estimation. Classification accuracy and angular error is reported on individual (20x20) grid locations. The angular error is calculated as the angular distance between the predicted and ground truth surface normal clusters. We report accuracies with and without binning.} }
\vspace{0pt}
\label{table:nyubin}
\noindent
\scalebox{0.75}{
\begin{tabular}{l|c|cc|c|cc}
%\begin{tabularz}{0.50\textwidth}{l |c *{6}{|Y}|}
\noalign{\smallskip}
& \multicolumn{3}{c|}{No Binning} & \multicolumn{3}{c}{Binned} \\
\hline
& (Higher Better) & \multicolumn{2}{c|}{(Error: Lower Better)} & (Higher Better) & \multicolumn{2}{c}{(Error: Lower Better)} \\
Net & Accuracy & Mean & Median & Accuracy & Mean & Median  \\
\hline
Agrawal et al. \cite{LSM2015} &  23.3 &  18.9 & 15.9 & 14.0 & 22.7 & 19.1  \\
Wang et al. \cite{cmuvideo}   &  18.0 &  21.3 & 18.9 & 10.5 & 23.6 & 24.7 \\
AlexNet                       &  25.4 &  18.8 & 14.2 & \textbf{17.6} & 21.6 & \textbf{15.3} \\ 
Random \scriptsize{(statistically informed)} &  9.2 &  25.0 & 24.9 & 5.0 & 27.2 & 25.2  \\
\hline
Ours &  \textbf{27.3} &  \textbf{17.7}  &  \textbf{13.5} &  17.4 & \textbf{20.7} & \textbf{15.3} \\
\hline
\end{tabular}}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
	\begin{center}
		\caption{\scriptsize{Evaluation of surface normal estimation on the NYU2 dataset using the common evaluation protocol affected by dominating wall, ceiling, and floor pixels. We used 1-NN technique on each representation to predict the normals. We report the pixelwise median error and the percentage of pixels that were within $11.5^{o}, 22.5^{o}$ and $30^{o}$ respectively. Our method outperforms the feature learning approaches of Agrawal et al \cite{LSM2015} and of Wang et al. \cite{cmuvideo} and is comparable to layer 7 features of AlexNet trained for Imagenet classification using this evaluation setup.}}. 
		\vspace{15pt}
		\label{table:nyu2}
		\begin{tabular}{l|c|c|c|c}
			\noalign{\smallskip}
			& (Lower Better) & \multicolumn{3}{c}{(Higher Better)} \\
			Net & Median & $11.5^{o}$ & $22.5^{o}$ & $30^{o}$ \\
			%\noalign{\smallskip}
			\hline
			Agrawal et al. \cite{LSM2015} &  20.2 &  29.1 &  54.5 &  67.9 \\
			Wang et al. \cite{cmuvideo} &  20.4 &  28.9 &  54.0 &  67.7 \\
			%AlexNet Pool-5 &  18.2 &  32.8 &  58.8 &  72.1 \\
			AlexNet &  19.7 &  30.3 &  55.7 &  69.5 \\
			\hline
			Ours &  19.6 &  30.7 &  55.6 &  68.8 \\
			%Joint Net (Ours) &  19.7 &  30.3 &  55.5 &  68.8 \\
			\hline
		\end{tabular}
	\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

\subsection{Prediction via Nearest Neighbors}

In addition to results presented above, we also used 1-Nearest Neighbor to compute the pixel wise surface normal errors. For each image in the test set, we found the closest image in the training set using each representation. The surface normals of this closest image were taken as the predicted surface normals for the query image. The pixel wise error in surface normal estimation for various CNNs is reported in Table \ref{table:nyu2}. The results are consistent with the experiments using a linear classifier.





==> tsnesup.tex <==



\section{Joint Embedding of Synthetic Cubes and Images}
In order to further investigate the nature our representations, we performed a joint tSNE embedding of synthetic cubes along with a single car category from the EPFL dataset (see Figure~\ref{fig:cubetsne}). This plot is closely related to the Cube$\leftrightarrows$Object nearest neighbor results provided in Figure 8 of the main paper (here we show all images but using a lossy 2D embedding; in Figure 8 of the main paper, the full dimensional representation was used for retrieving nearest neighbors, but only a few sample queries could be shown). 

If a representation mostly encodes semantic (or low level appearance) information, then cars and cubes should cluster into two different parts of the feature space, whereas if it encodes more geometric information, the organization should be based on pose. Figure \ref{fig:cubetsne} shows that our method embeds cubes and cars according to their geometric pose. In addition, in our feature space, cars and cubes are close together and one is enclosed by the other, whereas the baselines linearly separate them and put them far apart. This indicates that, as compared to other representations, ours predominantly capture geometric information over semantics or low-level appearance. It should be noted that synthetic cubes were sampled uniformly in the pose space, whereas cars in the EPFL dataset are not sampled uniformly (no camera pitch). Due to this, many cubes do not have a corresponding car and the tSNE plots are slightly skewed.  




\subsubsection{tSNE on Affinity Matrix:}
the tSNE embeddings in Figure~\ref{fig:cubetsne} are plotted in an affinity space. That is, given $N$ car and $M$ cube images, we compute the representation of each image and form a $(N+M) \times M$ affinity matrix where element $(i,j)$ is the $l_2$ distance between the representations of the $i^{th}$ image and $j^{th}$ cube. In other words, the representation of all of the car and cube images are cast based on the cube collection as the reference. We then perform the tSNE embedding on this $(N+M) \times M$ affinity matrix with each row being the $M$ dimensional representation of the image, rather than its original representation. 

We adopted this approach in order to enable the tSNE plots to bring out the geometric encoding aspect and not be dominated by the appearance/semantic information in the representation. For performing a successful pose estimation, encoding of both geometric and appearance information is essential~\footnote{For instance, if the pose estimation is being performed based on vanishing points, then besides extraction of at least 3  vanishing points from the input images, the correspondences among vanishing points needs to be done as well. Therefore, the representation must encode some appearance information in order to enable finding the correspondences among vanishing points.}. However, when a tSNE plot is formed, the user does not have any control over specifying whether the geometry or the appearance factor (or both) should govern the embedded space. In general, all of the manifolds existing in a representation contribute to the final 2D embedding. The workaround of finding the tSNE embedding on a unified affinity space lowers the impact of appearance as the appearance of all cubes are roughly the same while their pose covers a wide range. All of the plots in Figure~\ref{fig:cubetsne} (including the baselines) are formed using this approach. 

\begin{figure}
	\centering
	\includegraphics[width=0.64\textwidth]{figs/Cube_embed_v1.pdf}
	\caption{\scriptsize{tSNE embedding of the synthetic cubes and one category of EPFL dataset. Our representation shows a geometric organization while the baselines perform a clear semantic/appearance based separation.}}
	\label{fig:cubetsne}
\end{figure}



\section{Illustration of Pose Induction via tSNE Embeddings of more ImageNet Classes and MIT Places}

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1\textwidth]{figs/imagenettsne1.pdf}
	\caption{\scriptsize{tSNE of more ImageNet categories of our representation vs various baselines.}}
	\label{fig:imagenet1}
\end{figure*}


\begin{figure*}[h!]
	\centering
	\includegraphics[width=1\textwidth]{figs/imagenettsne2.pdf}
	\caption{\scriptsize{tSNE of more ImageNet categories of our representation vs various baselines.}}
	\label{fig:imagenet2}
\end{figure*}

We only trained our network for estimating 6-DOF pose on street view scenes. However, it appears that our representation learned something generic about the geometry of objects (see the discussion on unsupervised evaluations in section 4 of the main paper). This is elucidated by tSNE embeddings of objects in the Imagenet dataset (Figures~\ref{fig:imagenet1},\ref{fig:imagenet2}). These embeddings show that the feature space produced by our network performs pose induction for unseen object classes without any additional training.  

However it should be noted that a purely geometric approach is sometimes insufficient for a full object pose estimation, such as, distinguishing between front and back the car. Such knowledge is dependent on semantics and not merely geometry. It is therefore not surprising that our method puts such poses close to each other. In addition, one more mode of confusion of our method is putting together poses that are apart by 90 degrees. If the pose is indeed estimated based on vanishing points (see section 4.2 of the main paper), it is to be expected that objects 90 degrees apart in azimuth would have the same vanishing points and therefore it would require the knowledge of semantics to tease these poses apart. Since our method shows such confusion, it supplies further support that our method may performs pose estimation analogous to a method that would estimate pose based on vanishing points. 

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1\textwidth]{figs/mit_places_outdoorlib_v1_opt.pdf}
	\caption{\scriptsize{tSNE of our representation vs AlexNet (ImageNet) on a non-streetview dataset: MIT Places Benchmark (class `library' which is one of the pose rich categories). Our network shows a clear pose based embedding, unlike AlexNet trained on ImageNet. For both networks, the descriptor was computed over the entire image, and not patches.}}
	\label{fig:places}
\end{figure*}

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1\textwidth]{figs/wild_pose_7_opt.pdf}
	\caption{\scriptsize{This figure shows the same tSNE plot as the one in Figure~7 of the main paper, as well as AlexNet's tSNE for the sake of comparison. The AlexNet is trained on ImageNet and shows a non-geometric organization.}}
	\label{fig:wildposealex}
\end{figure*}

In addition to pose induction on imagenet, our method also performs pose induction on scene categories outside our street view dataset. For instance in Figure~\ref{fig:places}, the images of MIT places datasets (category library) are embedded according to pose. Finally, additional visualization of embedding of image patches from our dataset using our representation and AlexNet's (trained on Imagenet) are shown in Figure~\ref{fig:wildposealex}. 

\section{Additional Training Details}
For pose training we followed a curriculum strategy where we first trained only for angles within $[-90\degree, 90\degree]$ and then extended to all the angles. We found that this performed slightly better than directly training for all angles. 
We also experimented with employing quaternions, but found that predicting Euler angles performed better (quantitative results in the main paper). 


 

